Can I Solve It? Identifying APIs Required to Complete OSS Task

Open Source Software projects add labels to open issues to help contributors choose tasks. However, manually labeling issues is time-consuming and error-prone. Current automatic approaches for creating labels are mostly limited to classifying issues as a bug/non-bug. In this paper, we investigate the feasibility and relevance of labeling issues with the domain of the APIs required to complete the tasks. We leverage the issues' description and the project history to build prediction models, which resulted in precision up to 82% and recall up to 97.8%. We also ran a user study (n=74) to assess these labels' relevancy to potential contributors. The results show that the labels were useful to participants in choosing tasks, and the API-domain labels were selected more often than the existing architecture-based labels. Our results can inspire the creation of tools to automatically label issues, helping developers to find tasks that better match their skills.

==> background.tex <==
\section{Background}\label{sec:background}

In this section, we describe the background on skills in OSS and concepts of the multi-label classification approach used in this research.

\subsection{Skills on Open-Source Projects}\label{sec:Skill}

Several definitions can be related to our study. Firstly, ``skill'' is a particular ability a person developed after training and experience, a learned capacity, or a developed aptitude of doing something competently \cite{merriam-webster}. ``Knowledge'' can be abstracted, categorically represented, cataloged, and accessed \cite{faraj2000coordinating}. An expert is someone with special knowledge, skill, or training in something, whose level of performance exceeds most other \cite{merriam-webster}. ``Expertise'' can be defined as the skill of an expert \cite{mockus2002expertise} and refers to the characteristics, skills, and knowledge that distinguish experts from less experienced people \cite{ericsson2018cambridge}. 

SDExp \cite{baltes2018towards} is a theory of software development expertise grounded on data from a mixed-methods survey with Java and open-source software developers and in exiting literature on expertise and expert performance. According to concepts presented in SDExp, skills would be non-technical (as problem-solving, communication, continuous learning, and assessing trade-offs) and our study would be focused on finding the general and task-specific knowledge required for a developer to work on the project. However, following the concept that skill is as an ability someone developed after training and experience \cite{merriam-webster}, we are considering the technical abilities also as skills in this paper.

The relevance of knowing who has which knowledge and skill is the basis to design productive teams \cite{faraj2000coordinating}. A theory based on a survey with more than 300 open-source Java developers, and in existing literature on expertise and expert performance, concluded that an expert in software development should have skill for problem-solving, being able to break a complex problem into small pieces that can be solved to add back up to the whole. Besides, they should have other skills, as continuous learning, communication, understanding and implementing requirements, and being able to assess trade-offs when comparing alternative solutions \cite{baltes2018towards}.

Software development leaves traces of development activities in the repository, which can then be used for inferring the expertise of developers \cite{da2015niche}. In some domains, there is an objective metric for expertise, but in software development, there is no unique objective metric to predict how well a developer will solve a certain task \cite{mining_usage_expertise}. Moreover, if the person is a newcomer, there can be no historic data of his/her contributions to evaluate expertise. 

Based on this definitions, we positioned our study focusing on ``general'' skills that can be mapped to APIs knowledge required to solve an issue. If we can automatically label issues, we can provide context for a developer that is navigating through the project issues list trying to find an issue to work on. Thus, we hypothesize that developers can use their knowledge about themselves and decide which issues matches better with their APIs knowledge.

\subsection{Multi-label classification model}\label{sec:Skill}

Classification is one of the most techniques used nowadays to support several research areas. Basically, the classification is a predictive task that aims to predict a label  (or class) after creating a learning model from the labeled dataset. The most common approach is the binary classification that consists in finding a boundary able to separate the instances from the dataset into two groups, one belonging to the positive class and the other to the negative one \cite{MultilabelBook}.  

Different from the binary classification model, in a multi-label classification model \cite{6471714} each dataset instance is associated with a vector of classes, instead of only one class. Thus, the multi-label classification is a variant of the classification problem. Multi-label classification is also different from a multi-class classification problem when the classifiers have multiple classes to predict, but only one is associated with each instance \cite{MultilabelBook}.

To illustrate a multi-label classification scenario, we describe a common example: the movie multi-label genre classification. To build the model, a researcher/developer may use the summary or the legends of each movie as features to predict the genres associated with it. For instance, taking the Harry Potter and the Sorcerer's Stone\footnote{https://www.imdb.com/title/tt0241527/} in a hypothetical test set, the multi-label classifier must predict Adventure, Family, and Fantasy as genres (classes). However, is also important to avoid false positives genres predictions like romance, terror, or action. 

In practical terms, there are many approaches to employ multi-label classification \cite{MultilabelBook}. Basically, these approaches transform and decompose the multi-label classification into multiple binary classification problems.

In this paper, we employed two types of transformations (i) Binary Relevance and (ii) Classifier Chains. Binary relevance consists of training k classifiers, each for one label, taking the instances in which
the labels appear as positive and all the others as negative \cite{MultilabelBook}. The main drawback of Binary Relevance is that it does not take into account any label dependency and may fail to predict some label combinations if such dependence is present. However, Binary Relevance presents several advantages like learning methods can be taken as a base learner; it has linear complexity with respect to the number of labels, and it can be parallelized \cite{BinaryRelevance}.

A variation of Binary Relevance is to use the multi-label ensemble of binary classifiers, called Classifier Chains. Classifier
chains also train k classifiers, as many as labels there are in the dataset, choosing them in random order. The first classifier is trained using only the original input attributes. The first output label is then added as a new input attribute, and the new input space is used to train the second classifier, and so on. This way the classifiers are chained, taking into account the possible label dependencies \cite{MultilabelBook}.

In the following section we will present in more details the machine learning algorithms used and the evaluation metrics.

==> not_used.tex <==
Previous studies proposed different strategies to mitigate this problem, such as recommending tasks  \cite{anvik2011reducing,kevic2013collaborative,linares2012triaging}, finding experts to merge a pull request \cite{8716294}; identifying experts \cite{baltes2018towards, mining_usage_expertise, da2015niche, msr2019}; increasing engagement in code review discussions \cite{kavaler2018whom,ibrahim2010should} or reviewing and maintaining code \cite{thongtanunam2015should}. In general, the proposed strategies are useful for identifying experienced members based on their historical of previous contributions and interactions, and usually in the context of a single project. However, those strategies cannot help newcomers on matching their skills with the ones required by the project.

In this sense, it is worth mentioning that modeling skills in OSS is not an easy task. For instance, SDExp theory~\cite{baltes2018towards} defines that skills would be non-technical---like problem-solving, communication, continuous learning, and assessing trade-offs---which are very difficult to infer mining information from software repositories. 

While our focus is on helping developers to understand the required skills, we cornerstone on accurately predicting a subset of APIs, instead of having a comprehensive set of skills for each task. For instance, for a task that requires ``Database,'' ``User interface (UI,)'' ``Logging,'' and ``IO'', we nay be able to label the first three correctly, but not the fourth---because we did not have enough information to make the right prediction. We argue that even avoiding labeling some APIs, the contextual information provided by the labels will be useful to guide newcomers.

and its community 's community is very active and also involves the scientific community in general, and this is particularly interesting to our study since the onboarding process must consider contributors with no computer science background, who possibly face more challenges to chose their first task.


To support our conclusion, we performed the Kruskall Wallis statistical test together with the post-hoc Friedman chi-square statistical test. Both tests failed reject H\textsubscript{0.} to showing statistically significance in F-measure (Kruskall Wallis: p=0.866; Friedman test: p=0.152). The Friedman test showed that the precision values are significantly different when comparing the four models (Kruskall Wallis: p=0.586; Friedman test: p=0.002).  However, precision has contradictory results: Kruskall indicates fail to reject H\textsubscript{0} and Friedman indicating reject H\textsubscript{0.}

*** QUALITATIVE ABOUT DECISION MAKING TO PICK AN ISSUE *****

Suggestion: RQ1. How do contributors decide about what issue they will  work? RQ2. What information is used during the decision? RQ3. Why do they use this information? RQ4. What labels they would like the issue to have to help making this decision?

Our analysis of the answers revealed 21 categories that explain why our participants consider the information useful to help deciding. 5W2H is a flexible methodology that aims to assist in decision making and understanding what needs to be done to solve a problem \cite{fonseca2015utilization}. We organized the categories using the seven 5W2H dimensions (when, where, who, what, why, how, and how much), as can be seen in Figure \ref{fig:open_question1}. In the following, we present our findings organized by the 5W2H dimensions. The participants often provided an answer considering multiple aspects that were coded in more than one reason.

\begin{figure}[!htb]
\centering
\includegraphics[width=.48\textwidth] {images/open_question1.jpg}
\caption{Reasons presented by survey's participants to consider the information relevant to support their decision when choosing an issue to contribute}
\label{fig:open_question1}
\end{figure}

%The overall idea about the issue, issue details, issue status, issue goal, issue skills, issue level of difficulty, attempts to solve, user feeling about the issue, how to reproduce, how to debug, to feel safe to solve, issue kind, tips to address, issue documentation, the issue start point. 

From the 74 participants, 43 answered the open question Q2. "What kind of label would you like to see in the issues?", while 27 did not answer this question. We qualitatively analyzed the 43 answers, coded the different kinds of labels, and followed the same classification of Q1, grouping the codes into upper level categories using the 5W2H, i.e., when, where, who, what, why, how, and how much as we present in Fig. \ref{fig:open_question2}. There was no label cited by our participants related to why nor how much. The participants often provided an answer considering multiple aspects that we coded in more than one kind of label.

\begin{figure}[!htb]
\centering
\includegraphics[width=.48\textwidth] {images/open_question2.jpg}
\caption{Labels desired by survey's participants to support their decision when choosing an issue to contribute}
\label{fig:open_question2}
\end{figure}

****** OLD TABLE REASONS x REGIONS *****

\begin{table}[h!]
 \begin{center}
 \caption{Regions and Reasons}
 \label{tab:regionsResults}
\begin{tabular}{c|c} 
  \hline
  \textbf{Regions} & \textbf{Reasons}  \\
  \hline
Title &	\textbf{Overall idea, kind, level, goal, skill} \\
Tags and Labels	& \textbf{Kind, about}, tips, skill, match, \textbf{level} \\
Body &	\textbf{Details}, start point, about, level, \textbf{goal} \\
Comments & Safe, \textbf{details, attempts, kind, tips}, \\
         & start point, overall idea, \textbf{goal, level} \\
Code Snippet&	\textbf{Start point, details, debug} \\
Linked Issue &	\textbf{Status, documentation}, overall idea \\
Status &	\textbf{Status} \\
Participants & --- \\
 \hline
 \end{tabular}
 \end{center}
\end{table}

%We followed both qualitative and quantitative analysis to address the RQ2. 
%We created a classifier and used it to label the JabRef's issues according to the software architecture parts - that would be the technical skills a contributor should have to be able to work on the issue. Then, we cloned the JabRef's page of issues and presented to two groups of developers, asking them to rank three issues to contribute. In a follow-up set of questions.

%Regarding the question about what labels were relevant to support the decision to pick the three issues, we quantitatively analyzed the survey's responses of the two groups: who received the issues with only the original labels (control group) and who received the issues with both original labels and the labels generated by our classifier (treatment group). 

%The n-grams were obtained from the corpus using only the issue title because this simplest configuration performed better (small effect size) when we compared different corpus configurations. 

%The most mentioned reasons were: the overall idea about the issue, issue-level, and details. The overall idea covers the context of the problem or gives an introduction, while the level of difficulty helps the user to filter, and the details inform the user about the information available for one issue.

%Some quotes explained deeper the reasons: "The title was the most useful because it quickly introduced me to the issue. The title was the main thing I used to select my top 3. I wanted to make sure the title included something that wasn't too wordy and that it used words I could easily understand. I thought the tags or labels were also helpful. In particular the "good first issue" tag was very helpful, but it wasn't the most important thing for me when I was deciding my top 3." from P3N0, while P3C0 said, "Because I'm a beginner developer. The title and tags contributed with my choices."  P22I0 mentioned, "By filtering tags and labels I can search issues that I would like to contribute the most, as for the title and body I can grasp what's the idea of the issue, so I can better measure how long it would take to solve it. As for the comments I think it's easier since you can fully understand the issue and look for possible other solutions." and "familiarity with the code and tags helps to filter a lot through my area of expertise" (P16B0). P3B1 said, "I prefer backend X frontend, so I discarded issues with label "ui and the ones that seems to describe an interface problem/feature.  I prefer to work on bugs/performance issues and gave preference to those labels.". 

%\begin{table}[h]
% \begin{center}
% \caption{Analysis from same segments %regarding the API labels      
% - *N=API labels, O=old labels, T=Treatment C=Control }
% \label{tab:resultsRQ2Same}
% \begin{tabular}{c|c|r|r|r|r} 
%  \hline
%  \textbf{Group 1} & \textbf{Group 2} & %\textbf{$\chiˆ2$} & \textbf{p-value} & %%\textbf{Cramer's} &
 % \textbf{Odds} \\
 % \textbf{} & \textbf{} & \textbf{} & %\textbf{} & \textbf{V} &
 % \textbf{Ratio} \\
 % \hline
%ll N & All O & 23.6 & 1.158e-06 & 0.15 & 1.97 \\
%All T & All C & 1.41 & 0.23 & 0.031 & 0.87 \\
%INFNET N & INFNET O & 15.7 & 7.347e-05 & 2.92 & 3.83 \\
%INFNET T & INFNET C & 3.71 & 0.05 & 0.09 & 0.67 \\
%Blog N & Blog O & 18.0 & 2.202e-05 & 0.13 & 2.48 \\
%Blog T & Blog C & 1.77 & 0.18 & 0.5 & 1.35 \\
%CASNAV N & CASNAV O & --- & 0.51 & --- & 1.39 **\\
%CASNAV T & CASNAV C & --- & 0.002 & ---& 0.30 **\\
%  **  CASNAV used fischer test & & & & &//
%\hline
% \end{tabular}
% \end{center}
%\end{table}

%On the other hand, the analysis from the same segments had mixed results. Except for the CASNAV segment, all remaining did not show statistical significance between the treatment and control groups. However, when comparing the new and old labels in the same group, we found results statistically significant.


%Indeed, the low number of source code files where they are referenced likely indicates a proper project modularization, which can cause a low number of issues and consequently a lack of instances to improve the training set.
% MG: Isso pode ser tiro no pé. E se eles encapsularam em uma classe própria? A pessoa ainda precisa do conhecimento, mas não vai precisar alterar a class que encapsula a API. 

%Under the same segments (table \ref{tab:resultsRQ2Same} we could not claim a statistically significant difference between the API labels and the old ones in our data set, even though the odds ratio showed a 30\% minimum difference between them. However, when evaluating the API labels and the old labels together under the same segment and the same groups, we can see a statistical difference (except CASNAV) that should indicate a preference for these kinds of labels. 

%To solve that, we need to use a larger dataset with a representative number of those labels. This is probably a common situation in many projects when handling low-volume data for issues that are restricted to a few source codes.

%After three rounds, the patterns from question 47, "Why these pieces of information (regions) you select above in the previous question were useful?" converged, and 15 clusters arose. The same process was used to question 37, "What kind of label do you want to see in the issues?" where 10 clusters were found.

%We computed the odds ratio based on a 2x2 contingency table for each pair of respondent groups/segment (e.g., industry/students or treatment/control) and the number of relevancy/non-relevancy choices of a label.

%treatment and control groups from each available segment and next within the same segment 
%to understand their perceptions of the original labels and the labels generated by our classifier. 

%We collected data from 705 issues from the JabRef project and created labels to classify the APIs used in the source code. To determine the factors affecting the multi-label API classification, we investigated the influence of issue characteristics (title, body, and comments) to create the corpus and machine learning setup (n-grams and machine learning algorithms). Our best classifier used the Random Forest algorithm with issue title to create the corpus, uni-gram, and 899 tokens in the corpus. Using this model, we identified APIs with an average precision of 66\%, recall of 63\%, and an MCC of 0.55. More specifically, our results showed that, in general, five (``IO'', `UI'', ``Logging'', ``Test'', and ``Network'') of twelve labels evaluated can be predicted with 70\% of precision. 

%We randomly segregated all participants into two groups. One group received an issues' page with original labels and the other group received an issues' page with also the labels that our classifier included.

%Moreover, projects use several types of labels that can not be the ones containing the relevant information for a contributor to decide and pick an issue to solve.

%To address the limited space we keep the most important discussion on this paper and the remaining is available in the replication package.

%and (iii) a qualitative study with the developers and students who participated in the experiment to evaluate API labels in JabRef project and to derive directions to future work. 

%(i)~a method to automatically link issues to APIs;

%This paper target is to answer the following RQs:

%\MyBox{\emph{\textbf{RQ1: To what extent can a multi-label classification approach be used to predict the APIs required to work on existing tasks?}}} 

%The focus of the RQ1 is to explore the multi-label approach to automatically label the required APIs in JabRef issues. To help answer this research question, we investigated two factors: issues characteristics and machine learning comparison.

%Past research has employed text mining techniques using issue characteristics in different types of studies, such as bug prediction \cite{6899207}, change impact \cite{contextWiese}, software technology categorization \cite{NassifTech}, analysis of project README files \cite{ChristophReadme}, and issue lifetime prediction \cite{IssueLifetime}. Based on the previous research, we use issue characteristics---such as title, body, and comments---to investigate each piece of information’s influence in predicting the API required to solve a task. From a practical perspective, two aspects are essential: (i) using only the title is better than aggregating all the information, since adding new sources of data can increase the data collection and data pre-processing effort; (ii) by using the characteristics of the issues, we can develop a way to automatically label new issues with their required API as soon they are reported in the project repository and (iii) how the machine learning algorithms influences the prediction results. Our experiments were based on a similar method used by Beyer et al., \cite{MachineLearning}, who used multi-label classification approach to predict question categories in SO. It is essential to highlight that if one can accurately create classification models, only using the issue title is better than using all the information combined, since some issues lacked some information \cite{zimmermann2010makes,Bettenburg:2007:QBR:1328279.1328284,vaz2019empirical}.

%The second group of hypotheses investigates how the machine learning algorithms influences the prediction results. Our experiments were based on a similar method used by Beyer et al., \cite{MachineLearning}, who used multi-label classification approach to predict question categories in SO. 

%\MyBox{\emph{\textbf{RQ2: To what extent labeling issues with APIs helps developers to select the issues to contribute?}}} 
 
%The RQ2 aims to confirm the claims from the quantitative study, that API labels can help the contributors and the corpus used to mine the data set is perceived as important from the developer's perspective. 

%The number of complete responses (the only ones we considered for the analysis) was divided in students and practitioners from the industry. 

%The participant was asked to look at the issues and select three issue to contribute. After clicking on the issue, we presented an issue's form divided in regions, and asked the participant to click to mark the regions that helped him to chose that issue. 



%To analyze the results, as the data was independently collected and cannot be paired, a chi-square test ($\chi^2$) was used to determine if the data for the two groups are statistically different. The standardized effect size of the $\chi^2$ test was calculated using the Cramer’s V statistic.




%4. Pages with labels (original and classifier-based) present in the selected issues, to identify which ones were relevant in the selection of issues. To the treatment groups we presented the API labels generated by the classifier and the original labels. To the control group only the original labels were visible. We selected the labels with more True Positive and False Negative results we considered the best indicators of a good and bad results, respectively. Thus the set of labels were "UI", "IO", "Logging", "Test", "OS", "Google Common", "Database" and "Network".

%, was grouped in 10 different types: priority,	architecture	issue kind, hard skills related to, issue status, issue API/Library, issue goal, issue tips, issue-level, and GitHub info related to the issue. The most requested labels were hard skills, priority, and kind with 15, 10, and 9 options. The hard skills include programming languages and frameworks. The priority tag shows if the issue is a minor or major or impacts the operation. The kind labels explain if the issue is a bug, feature, or overall idea about the problem. For example, P9B1 mentioned, "One that indicates that the issue is critical/important, and labels related to technologies/frameworks/libs involved",  was classified as "priority", "hard skills" and "API". Another example was "Maybe an information about programming language or if it is related to frontend, backend or database" (P7B1) was classified as hard skills and architecture.

%We employed the research method to achieve the main goal of this work: To understand whether API labels can help  developers to decide for an issue to contribute. 
%In Phase 1, we collected data from JabRef project using GitHub API. We also cleaned the data collected from issue, pull requests and source code. In phase 2, we created the corpus using data previously filtered in Phase 1. In this phase, we stemmed the corpus, removed the stop words, applied the TF-IDF) and also selected the algorithms and quantitatively evaluated the multi label classification. In phase 3, we carried out an experiment with developers with subsequent data collection using a survey.

%\textbf{What labels do users want to see?} 42 participants from 74 answered the open question Q2: ``What kind of label do you want to see in the issues?''. Many different semantics appeared. It seems, technology, priority and types are the most important ones. For example, P9B1 mentioned, \textit{``One that indicates that the issue is critical/important, and labels related to technologies/frameworks/libs involved''}. Another example was \textit{``Maybe an information about programming language or if it is related to frontend, backend or database''} (P7B1)
%as suggested by P10P1: \textit{``impact on operations.''}. 
%However UX aspects are important to addreess when labeling as P3B1 mentioned: \textit{``I thought it's important to only put relevant'' labels on the issues, 'cause improving the number of label could make them less readable.''} 
%The word ``type" appeared repeatedly as the desirable label in quotations. \textit{``type: performance, type: feature, API: User Interface and type: enhancement''} answered P12B0, while P8B1 said \textit{``Labels that can define the type of the problem''} and \textit{``The type of the programming language''} (P11P1). Indeed, "types" seems to have many possible semantics and must be better explored in future work.   


%\textbf{Reasons to consider the information relevant} From the 74 participants who finished the survey, 47 answered the open question Q1. ``Why the information you selected was relevant?'' and 27 did not answer. 
%Many suggested the relevance of the labels, like P5B0, P4B0 (Tab: \ref{tab:reason_Open}). While P4B0 considered the \textsc{Labels} less relevant than the \textsc{Title}, others said the \textsc{Labels} are the fastest way to have a overall idea about the skills required to solve the skills (e.g. P13I0, P13B0 and P14B0). 
%We present some of the participants' quotes in Table \ref{reason_Open}.

%\subsubsection{Segmented Analysis}

%In this section, we look deeper into the results to understand the prevailing preferences for regions of information inside the issue page and preferences for labels among our participants and across different demographics.

%The statistical analysis from the different demographics used the chi-square test. The result indicates that the number of relevant labels is significantly different between all demographics (industry and students, experienced and novice developers, OSS contributors and non-contributors, and who has and has not affinity with the JabRef's technology) with small effect sizes. The only exception was when comparing the all dataset using treatment and control groups where did not result in statistical significance.


%The  most  selected  issues  were  4306,  3994  and  the  4977 with 25, 22 and 18 selections followed closer by 4233, 5679 and 5002 figure (\ref{fig:issuechoices}). %The reasons for selection used for the top 3 issues were shown in table \ref{tab:reasons_regions} in bold.

%However UX aspects are important to address when labeling as P3B1 mentioned the problems created by a possible label overhead. The word ``type'' appeared repeatedly as a desirable label in quotations. P12B0,  P8B1 and P11P1 are examples. Indeed, "types" seems to have many possible semantics and must be better explored in future work.   


%RQ2
%Here is an overview of the issues that participants selected: 
%We presented the regions of the issue's information page and asked the participant to mark which of them are relevant to decide taking the issue, then open asking why. We also listed the labels they had in the issues' page - the control group had the issues' page only with the original labels and treatment group had also the labels generated by our classifier - and asked which of them were relevant to decide selecting the issue.

%First of all, we compared the set of issues selected and the information used by participants to choose the task to work on in the treatment group and control group.

%We split the participants into two groups: one that had access to the new labels (treatment group) and other that did not (control group).

%Analyzing the most selected issues can reveal preferences for some types of issues, combining information about the title, labels types, number of labels, comments size, presence of images or code snippets etc. 
%In general, the issues selected by participants from all subgroups were the same: 4306, 3994, 4977, and 4233. % (Tab. \ref{tab:issuesCountsSegments}). %The issue 4306 was chosen by 15 (36.5\%) participants in treatment group and 10 (30.3\%) control. 3994 receive 12 (29.3\%) selections from treatment and 10 (30.3\%)from control and 4977, 11 (26.8\%) from treatment and 7 (21.2\%) from control. %Issue 4306 contains the API labels ``UI'', ``IO'', ``Test'', ``Good First Issue'' four labels in the six most selected in treatment. But only one in the five most selected labels control group: ``type: enhacement''. Issue 3994 contains ``UI'', ``IO'', ``DB'', ``type:bug'', four in the six most selected in treatment, and the most selected in the control group. Issue 4977 contains ``UI'', ``IO'', ``Test'', ``Good First Issue'' the most selected two labels in treatment and the most in control. 
%Some of these issues received different selections: 4233 was mostly selected by the most experienced developers. The same occurred with 3994. Issue 4997 yielded small differences, and 4306 was always selected by the subgroups with less experience. Both (4997 and 4306) contained the label ``Good First Issue''. Three were manually labeled with the ``type:bug'' labels and all of them with the ``UI'' API label. But other labels with the same labels did not receive the same attention. Two had figures (showing user interfaces) in the issue page, two had code snippets, two had many comments, and two had only a few comments. Finally,  628 was almost never selected by the subgroups with more experience even with the most selected labels present. The issues 2319 and 2370 were selected few times, despite they have the most selected labels. (Fig. \ref{fig:issuechoices}). Thus, no pattern was evident in our analysis, suggesting that the selection process relies on a complex set of information.

%5679 the fifth most chosen (treatment, control) = (10,4) (24.4\%,12.1\%), 5254  (1,5) (2.4\%,15.1\%), 4360 (4,1) (9.8\%,0.3\%), 2319 (0,5) (0\%,15.1\%) and 2370  (3,1) (7.31\%,3\%). 5679 and 4360 were unlabeled in control group and had only API labels (treatment). They are the only two cases of unlabeled issues.

%\input{tables/issuesCountsSegments}

%\begin{figure}[!hbt]
%\centering
%\includegraphics[width=.4\textwidth, trim= 50px 45px 50px 40px] %{images/issuesCountsTC.png}
%\caption{\newline Number of choices by issues treatment and control groups ordered}
%\label{fig:issuechoices}
%\end{figure}

%\begin{figure}[!hbt]
%\centering
%\includegraphics[width=.4\textwidth, trim= 50px 45px 50px 40px] {images/issuesCountsSegments.png}
%\caption{\newline Number of choices by issues by subgroups normalized}
%\label{fig:issuechoices}
%\end{figure}

%\textbf{What the most relevant information (regions) for all participants when selecting an issue?}


%We found that participants' preferences matched with the results obtained in RQ1, given the observation that issue title was the best feature for creating the classifiers.

%\textbf{Are the most relevant information (regions) different between the control and treatment groups?}
%Next, we investigated whether the regions in issue pages differed in relevance by the treatment and control groups. This can indicate whether the API Labels increased the importance of the label's regions on pages. 
%When comparing the regions' relevancy in treatment and control groups, considering label and other regions, we did not find any statistical difference ($chiˆ2$- = 2.3537, df = 1, p-value = 0.125). 

%\textsc{Title} was considered relevant because it makes it possible to \textit{``quickly think about the efforts needed to take a task''} (P3CT). The \textsc{Title} also attracted participants for its usefulness in picking an issue to solve (P10IT, P3NC, P14BT) and for trying to match their skills  \textit{``seeing whether or not being capable of finding a solution"} (P4BC). %However, there is need for caution when filling the title, as \textit{``title must match with the issue''} (P6BT). Otherwise, this important region of information was considered useless, and a contributor \textit{``mostly will not look at the title because people tend to give bad titles to issues, what they really want or need we be at the body''} (P7B0). 

%\textbf{API labels are playing a role to choose the issues?} 
%Both groups selected the \textsc{Type Bug} as the most relevant label to decide about selecting an issue to contribute. However, after this first selection, the treatment group selected three API labels generated by our classifier (\textsc{UI}, \textsc{Test} and \textsc{Database}), and the control group selected \textsc{Type Performance}, \textsc{Type Quality} and \textsc{Type Feature} as the most relevant labels to make the decision.

%Considering the demographic subgroups, we compared the relevance of the generated labels. Table \ref{tab:resultsRQ2Dif} shows that p-values for all demographics are below the significance threshold ($<$0.05), rejecting the chi-square independence test null hypothesis and indicating no relationship between the demographic subgroups with a small effect size (Cramer's V varying from 0.13 to 0.21). This result means the demographic subgroups had different results and perceptions about the relevance of the generated API labels i.e., they chose the API labels in a different way. Comparing the table \ref{tab:resultsRQ2Dif} and the Figs. \ref{fig:newlabels_countsAC} \ref{fig:newlabels_countsAT} we can observe the subgroups with more experience (industry, experienced coders, experienced OSS Contributors, and participants with high experience with JabRef technologies), selected the API labels more often with only two exceptions, ``OS'' was more selected by students and ``Test'' was more selected by participants with low experience with JabRef's technology. This result might suggest the perception of the API labels is higher when the participant has more experience. 

%Finally, looking to some labels among the demographic subgroups, it is possible to observe some patterns. ``UI'', ``DB'' and ``IO'' are always more often selected by the experienced subgroups, and they are the three most selected API labels in the top four. These findings support the importance of these labels to contribute to the JabRef project.

%Fig, \ref{fig:newlabels_countsIS}, shows the API labels selected by the demographics subgroups.


%Finally we looked to the four most select labels as relevant, what would help contributors to select an issue, three are API labels (Fig.\ref{fig:labels_counts} treatment counts). The same labels were the three most relevant API labels selected, considering all subgroups (\textsc{UI}, \textsc{Test}, and \textsc{Database}).  %The remaining subgroups had similar results showing proportional more API labels selections in Experienced Coders, OSS Contributors and High Experience subgroups. 


%\begin{figure}[!htb]
%\centering
%\includegraphics[width=.48\textwidth] {images/newLabelsCountsIndStu.png}
%\caption{The API labels selected as most relevant by participants from Students and the Industry subgroups ordered by the relevancy counts.}
%\label{fig:newlabels_countsIS}
%\end{figure}

%\begin{figure}[!htb]
%\centering
%\includegraphics[width=.48\textwidth] {images/indStuCounts3x1.png}
%\caption{The labels selected as most relevant by industry and students participants ordered by the relevancy counts normalized.}
%\label{fig:newlabels_countsIS}
%\end{figure}



%\begin{figure}[!htb]
%\centering
%\includegraphics[width=.48\textwidth] %{images/violinAPIxCompZero.png}
%\caption{Density Labels API x Components.}
%\label{fig:newlabels_countsACZ}
%\end{figure}

%\begin{figure}[!htb]
%\centering
%\includegraphics[width=.48\textwidth] %{images/violinAPIxTypeZero.png}
%\caption{Density Labels API x Type.}
%\label{fig:newlabels_countsATZ}
%\end{figure}


%\begin{figure}[!htb]
%\centering
%\includegraphics[width=.48\textwidth] {images/indStuNewOldCounts.png}
%\caption{Sum labels selected as most relevant by industry and students participants normalized.}
%\label{fig:newlabels_countsIS}
%\end{figure}

%\begin{figure}[!hbt]
%\centering
%\includegraphics[width=.4 \textwidth, trim= 50px 45px 50px 40px] {images/hotSpotCountsTop3.png}
%\caption{The regions of the issue's information page selected as most relevant by participants from both groups and from the top 3 selected issues.}
%\label{fig:hotmapchoicestop3}
%\end{figure}


%\input{tables/label_types.tex}

%\textbf{What labels do users want to see?} 42 participants (out of 74) answered the open question Q2 (``What kind of label do you want to see in the issues?''). The \textsc{type}, the \textsc{priority} to solve, and the \textsc{programming language} \textit{``in which the code was written in"} (P3N0) were the three most mentioned, followed by the \textsc{difficulty level} and the \textsc{architecture layer}. 
%Some participants suggested different semantics for the label \textsc{Type}: bug (P13B0, P7B0), improvement (P13B0), performance (P11B0, P12B0), new feature (P12B0), or security (P7C0). Other participants also suggested different semantics for \textsc{Difficulty Level}: \textit{``good first issue"} (P14I0), \textit{``good challenging issue"} (P3C0), or \textit{``easy, medium, hard"} (P14B0). The semantics for each label can be explored in future work. We present the 11 categories of suggested labels that we qualitatively coded from the participants answers in Table \ref{tab:desired_labels}.

%\input{tables/desired_labels}



%We group the related work by task recommendation, expertise, automatic tagging, and APIs.

%\textit{Task Recommendation}. Previous work reports the challenges that newcomers face in finding an appropriate task to start. Among these challenges for newcomers, the following stand out: identifying bugs that are interesting to them; finding tasks that match with their skill sets; and the risk of starting to work on a stale or duplicate task \cite{Wang.Sarma_2011,HICCSTask}. 

%In contrast, studies showed that README files \cite{Readme} and contribution guidelines \cite{8919187} are not always complete and did not match the contribution process.

%Although some communities expect new developers to find tasks to work \cite{vonKrogh}, the literature explores strategies and challenges for task recommendation in OSS projects. These strategies rely on extensive manual work to tag the issue tracker system (ITS) and do not consider newcomers' skills. In this work, we propose an approach to automatically label APIs required in open source issues, to provide more contextual information to help newcomers in their decision to choose a task. 

%\textit{Expert Identification}. Regarding the identification of experts, the literature presents techniques based on general metrics, such as developer's interests (e.g., what they program in their free time) and technical skill (e.g., programming languages they are using) \cite{greene2016cvexplorer}, developer's activity from Stack Overflow (SO) and GitHub \cite{huang2016cpdscorer}, and individual's performance on a set of programming tasks~\cite{bergersen2014construction}. On the other hand, some techniques use traces from source code ~\cite{msr2019,da2015niche}, bug report data ~\cite{anvik2011reducing}, and merging pull requests data ~\cite{8716294} to rank developers who are the most appropriate to review code, merge a pull request, or even comment on an issue. The work of \cite{vadlamani2020studying} aims to understand why developers contribute to GitHub and SO. 

\author{\IEEEauthorblockN{Fabio Santos,\textsuperscript{$1$} Igor Wiese,\textsuperscript{$2$}  Bianca Trinkenreich,\textsuperscript{$1$} Igor Steinmacher,\textsuperscript{$1,2$} Anita Sarma ,\textsuperscript{$3$} Marco A. Gerosa, \textsuperscript{$1$}}

\IEEEauthorblockA{\textsuperscript{$1$}\textit{Northern Arizona University, USA}, \textsuperscript{$2$}\textit{Universidade Tecnológica Federal do Paraná, Brazil},  \textsuperscript{$3$}\textit{Oregon State University, USA}
\\ 
\\
\{Fabio-Marcos.De-Abreu-Santos,bt473,marco.gerosa\}@nau.edu\textsuperscript{$1$}, \{igorfs,igor\}@utfpr.edu.br\textsuperscript{$2$}, anita.sarma@oregonstate.edu\textsuperscript{$3$}}
}


==> tables/APILabelsTablesOdds.tex <==
\begin{table}[h]
 \begin{center}
 \caption{Analysis from different segments regarding the API labels 
 - *N=API labels, O=old labels, T=Treatment C=Control, A=all labels}
 \label{tab:resultsRQ2Dif}
 \begin{tabular}{c|c|r|r|r|r} 
  \hline
  \textbf{Group 1} & \textbf{Group 2} & \textbf{$\chiˆ2$} & \textbf{p-value} & \textbf{Cramer's} &
  \textbf{Odds} \\
  \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{V} &
  \textbf{Ratio} \\
  \hline
N:Industry & Students & 7.15 & 0.007 & 0.14 & 1.82 \\
A:Industry & Students & 6.41 & 0.01 & 0.06 & 1.31 \\
N:E. coders & Non E. coders & 15.53 & 8.08e-05 & 0.20 & 2.82 \\
A:E. coders & Non E. coders & 9.4 & 0.002 & 0.07 & 1.4 \\
N:Contrib & Non Contrib & 14.17 &  0.0001 & 0.19 & 6.58 \\
A:Contrib & Non Contrib & 11.34 &  0.0007 & 0.08 & 1.72 \\
N:Affinity & No Affinity & 6.55 &	0.01 & 	0.13 &	1.80 \\
A:Affinity & No Affinity & 4.12 &	0.04 & 	0.05 &	1.24 \\
All N & All O & 23.6 & 1.158e-06 & 0.15 & 1.97 \\
All T & All C & 1.41 & 0.23 & 0.031 & 0.87 \\
\hline
	
 \end{tabular}
 \end{center}
\end{table}

==> tables/APILabelsTreatment.tex <==
\begin{table}[h]
 \begin{center}
 \caption{$chi^2$ and Cramer's V analysis from different demographic subgroups regarding the API labels}
 \label{tab:resultsRQ2DifTreatment}
 \begin{tabular}{c|c|r|r|r} 
  \hline
  \textbf{Groups} & \textbf{Labels} & \textbf{$\chiˆ2$} & \textbf{p-value} & \textbf{Cramer's V} \\
  \hline


Industry/Students & API/Comp & 0.02 & 0.87 & 0.009\\
Industry/Students & API/Type & 0.14 & 0.70 & 0.02 \\

Exp/Novice Coders & API/Comp & 0.02 & 0.86 & 0.01  \\
Exp/Novice Coders & API/Type & 2.46 & 0.11 & 0.08  \\


\hline
	
 \end{tabular}
 \end{center}
\end{table}

==> tables/APIlabelsOld.tex <==
\begin{table}[h]
 \begin{center}
 \caption{Analysis from different segments regarding the API labels 
 - *N=API labels, O=old labels, T=Treatment C=Control, A=all labels}
 \label{tab:resultsRQ2Dif}
 \begin{tabular}{c|c|r|r|r} 
  \hline
  \textbf{Group 1} & \textbf{Group 2} & \textbf{$\chiˆ2$} & \textbf{p-value} & \textbf{Cramer's} \\
  \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{V}  \\
  \hline
N:Industry & Students & 7.15 & 0.007 & 0.14  \\
A:Industry & Students & 6.41 & 0.01 & 0.06  \\
N:E. coders & Non E. coders & 15.53 & 8.08e-05 & 0.20  \\
A:E. coders & Non E. coders & 9.4 & 0.002 & 0.07  \\
N:Contrib & Non Contrib & 14.17 &  0.0001 & 0.19  \\
A:Contrib & Non Contrib & 11.34 &  0.0007 & 0.08  \\
N:Affinity & No Affinity & 6.55 &	0.01 & 	0.13  \\
A:Affinity & No Affinity & 4.12 &	0.04 & 	0.05  \\
All N & All O & 23.6 & 1.158e-06 & 0.15  \\
All T & All C & 1.41 & 0.23 & 0.031  \\
\hline
	
 \end{tabular}
 \end{center}
\end{table}

==> tables/APIxCompxTypeTreatment.tex <==
\begin{table}[h]
 \begin{center}
 \caption{Answers from different demographic subgroups regarding the API labels}
 \label{tab:apiXcompXtypeTreatment}
 \begin{tabular}{c|c|r|r} 
  \hline
  \textbf{Subgroup} & \textbf{Comparison} & \textbf{\%} & \textbf{\%} \\
  \hline

Industry & API/Comp & \textbf{66.8} & 33.2 \\
Students & API/Comp & \textbf{68.5} & 31.5 \\


Exp. Coders & API/Comp & \textbf{66.3} & 33.7 \\
Novice Coders & API/Comp & \textbf{68.1} & 31.9  \\

Industry & API/issue Type & \textbf{54.8} & 45.2 \\
Students & API/issue Type & \textbf{52.1} & 47.8 \\


Exp. Coders & API/issue Type & \textbf{60.4} & 39.6 \\
Novice Coders & API/issue Type & \textbf{50.8} & 49.2  \\

\hline
	
 \end{tabular}
 \end{center}
\end{table}

==> tables/APixCompxType_old.tex <==
\begin{table}[h]
 \begin{center}
 \caption{Answers from different demographic subgroups regarding the API labels}
 \label{tab:apiXcompXtype}
 \begin{tabular}{c|c|r|r} 
  \hline
  \textbf{Subgroup} & \textbf{Comparison} & \textbf{\%} & \textbf{\%} \\
  \hline

Industry & API/Comp & \textbf{56.0} & 44.0 \\
Students & API/Comp & 40.0 & \textbf{60.0} \\

Exp. Coders & API/Comp & \textbf{50.9} & 49.1 \\
Novice Coders & API/Comp & 41.5 & \textbf{58.5}  \\

Industry & API/issue Type & 45.5 & \textbf{55.5} \\
Students & API/issue Type & 30.6 & \textbf{69.4} \\

Exp. Coders & API/issue Type & 43.5 & \textbf{56.5} \\
Novice Coders & API/issue Type & 30.9 & \textbf{69.1}  \\

\hline
	
 \end{tabular}
 \end{center}
\end{table}

==> tables/demoWithTreatment.tex <==
\noindent\textbf{Comparison between API Labels and component}
Practitioners select marginally less API labels than students (66.8\% x 68.5\%). And practitioners select marginally more components labels than students (33.2\% x 31.5\%).

The same occurred when we compared the experienced and novice coders: more API labels preference from experienced coders (66.3\% x 68.1\%). And marginally more component labels from experienced coders (33.7\% x 31.9\%).

API labels were \textbf{more} selected than component with similar results from the industry (66.8\% x 33.2\%) and experienced (66.3\% x 33.7\%). The student (68.5\% x 31.5\%) demographic subgroup and the novice (68.1\% x 31.9\%) coders subgroup also had similar selections for the component labels.

\noindent\textbf{Comparison between API Labels and issue type}
Practitioners also selected more API labels (54.8\% x 52.1\%) than students and less issue type labels (45.2\% x 47.8\%) as well. And experienced coders selected more API labels than novice (60.4\% x 50.8\%) and less issue type than novice coders (39.6\% x 49.2\%).

API labels were \textbf{more} selected than issue type with a difference between industry (54.8\% x 45.2\%) and experienced (66.3\% x 33.7\%). The student (52.1\% x 47.8\%) demographic and the novice (50.8\% x 49.2\%) coders subgroup had similar selections for the issue type.

It suggests the API labels are perceived with more relevant a great difference from all subgroups than the component labels.  API labels also were perceived more relevance than the issue types with a marginal difference in the subgroups, except in the experienced coders where we could observe a greater difference.
\input{tables/APIxCompxTypeTreatment}

Table \ref{tab:resultsRQ2Dif} shows that p-values for all demographics are over the significance threshold ($>$0.05). 

The null hypothesis, states there is no significant difference between the expected and observed result, and here it means the two groups have the same distribution. So, the proportion of practitioners group and the students comparing the API labels to component labels is not significant, and $chi^2$=0.02, p=0.87,  with a small effect size (Cramer's V = 0.009). Comparing API labels to issue types we also did not observed a difference in proportions with $chi^2$=0.14, p=0.70, with small effect size (Cramer's V =0.02). Comparing the experienced coders and novice, there is not a difference in proportions from the API labels to the issue types, ($chi^2$=0.02, p=0.86) with a small effect size (Cramer's V =0.-1), and there is no difference in proportions comparing the API labels and the component labels ($chi^2$=0.11, p=0.08).

\input{tables/APILabels}

\MyBox{\textbf{\emph{RQ2 Summary.}} Our findings suggest that Title and Labels have important information for selecting an issue to work. API labels regions also increased the perception of the label region's relevancy. Comparing the demographic subgroups industry and experienced coders selected more and with same distribution the API labels than the Component labels and isue types. \XXX}

\section{Discussion}

This section discuss our results and future work. 

\noindent\textbf{Are API labels relevant?} The Table \ref{tab:resultsRQ2Dif} indicates how each demographic subset perceived the API labels' relevancy. Comparing with the component labels and issues types, all subgroups selected more the API labels and it might suggest a preference for the API labels. Our first insight was that the API labels could help newcomers, and could be more selected by the subgroups with less experience by providing them with more information to make a decision, but the result might suggest a more embracing preference for the API labels including experienced coders and those who work in the industry. %It might indicate the more the developer is closer to the project's technical skills, %or to the technology in the scope of this survey, 
%the more important it is to have detailed information about the API to solve an issue. 
This study enriches the previous literature (\ref{sec:related}) by adding new contextual information for developers that are trying to onboard to a new project. On the other hand, new hypotheses may be investigated to explore in depth the type of technology fit for labeling in the appropriate granularity. Those topics can be explored in a future work. 

It is also important to better investigate what will be most effective for helping new contributors in onboarding. In fact, one participant (P3BC) mentioned that ``UX aspects are important to address when labeling, pointing to the problems created by a possible label overhead''. 

\section{Conclusion}

We found all demographic groups select more the generated labels suggesting the API labels' relevance, comparing with the component labels.



Finally ,treatment group select  API labels more than component labels with a statistical difference, confirming our claim above about their usefulness.

==> tables/demographics.tex <==
\begin{table}[]
\begin{tabular}{ccccccc}
\cline{1-3}
\multicolumn{1}{|c|}{\textbf{Role}}           & \multicolumn{1}{c|}{\textbf{\#}} & \multicolumn{1}{c|}{\textbf{\%}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{Affinity with JabRef technology} & \multicolumn{1}{c|}{\#} & \multicolumn{1}{c|}{\%} \\ \cline{1-3}
\multicolumn{1}{|c|}{Practitioner}            & 41                               & 55.5                             & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{High Affinity}                   & 31                      & 42                      \\ \cline{1-3}
\multicolumn{1}{|c|}{Student}                 & 33                               & 44.5                             & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{Low Affinity}                    & 43                      & 58                      \\ \cline{1-3}
                                              & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}                                 & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}    \\ \cline{1-3}
\multicolumn{1}{|c|}{Experience as Developer} & \multicolumn{1}{c|}{\#}          & \multicolumn{1}{c|}{\%}          & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{Experience as OSS Contributor}   & \multicolumn{1}{c|}{\#} & \multicolumn{1}{c|}{\%} \\ \cline{1-3}
\multicolumn{1}{|c|}{Experienced}             & 28                               & 38                               & \multicolumn{1}{l|}{}          & \multicolumn{1}{c|}{Experienced}                     & 10                      & 13.5                    \\ \cline{1-3}
\multicolumn{1}{|c|}{Novice}                  & 46                               & 62                               & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{Novice}                          & 64                      & 86.5                    \\ \cline{1-3}
\end{tabular}
\end{table}

==> tables/desired_labels.tex <==
\begin{table}[htb]
\centering
\caption{Labels desired by participants to select the issue}
\label{tab:desired_labels}

\begin{tabular}{|c|c|}
\hline
Desired Labels     & Participants who mentioned              \\ \hline
type &
  \begin{tabular}[c]{@{}c@{}}P7B0, P11B0, P12B0, P13B0, P7C0, P8B1, P8P1\\ P4C1, P5N1, P21I1\end{tabular} \\ \hline
priority &
  \begin{tabular}[c]{@{}c@{}}P3B0, P11I0, P22I0, P9B1, P5P1, P10P1, P15I1\\ P16I1, P17I1, P3N1\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}programming \\ language\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}P10B0, P13I0, P3N0, P6B1, P7B1, P3P1, P11P1\\ P22I1, P23I1\end{tabular} \\ \hline
difficulty level   & P14B0, P21B0, P14I0, P3C0, P10I1, P11I1 \\ \hline
technology         & P6B0, P10B0, P13I0, P4B1, P9B1, P18B0   \\ \hline
architecture layer & P4B0, P13B0, P7B1, P3N1                 \\ \hline
API                & P7B0, P12B0, P13B0, P7P0                \\ \hline
status             & P5B0, P10I1, P16I1                      \\ \hline
GitHub info        & P10P0, P22I0                            \\ \hline
database           & P13I0                                   \\ \hline
framework          & P9B1                                    \\ \hline
library            & P9B1                                    \\ \hline
\end{tabular}
\end{table}



==> tables/issuesCountsSegments.tex <==
\begin{table}[h]
\begin{center}
\caption{Percents of the most selected four issues by subgroups}
\label{tab:issuesCountsSegments}
\begin{tabular}{lllll}
  \hline
     \textbf{Subgroups}                & \textbf{4306} & \textbf{3994} & \textbf{4977} & \textbf{4233} \\
\hline
Industry             & 0.30 & 0.30 & 0.24 & 0.37 \\
Students             & 0.37 & 0.29 & 0.24 & 0.15 \\
Experienced Coder    & 0.25 & 0.39 & 0.29 & 0.39 \\
Novice Coder         & 0.39 & 0.24 & 0.22 & 0.13 \\
Exp Contributor      & 0.20 & 0.40 & 0.20 & 0.60 \\
Novice Contributor   & 0.36 & 0.28 & 0.25 & 0.17 \\
High Exp JabRef Tech & 0.26 & 0.32 & 0.32 & 0.36 \\
Low Exp JabRef Tech  & 0.40 & 0.28 & 0.19 & 0.14 \\
  \hline
 \end{tabular}
 \end{center}
\end{table}

==> tables/label_types.tex <==
\begin{table}[]
 \caption{Quotations about the API labels Types}
 \label{tab:labelTypes}
\begin{tabular}{c|l}
\hline
Participant & \multicolumn{1}{c}{Quotation} \\
  \hline 
P9B1        & \begin{tabular}[c]{@{}l@{}}\textit{``One that indicates that the issue is critical/important, }\\ \textit{and labels related to techs/frameworks/libs involved''}\end{tabular}                         \\
P7B1        & \begin{tabular}[c]{@{}l@{}}\textit{``Maybe an information about programming language or }\\ \textit{if it is related to frontend, backend or database''}\end{tabular}                                         \\
P10P1       & \textit{``impact on operations.''}             \\
P3B1        & \begin{tabular}[c]{@{}l@{}}\textit{``I thought it's important to only put relevant'' labels on }\\ \textit{the issues, 'cause improving the number of label could} \\ \textit{make them less readable.''}\end{tabular} \\
P12B0       & \begin{tabular}[c]{@{}l@{}}\textit{``type: performance, type: feature, API: User Interface and} \\ \textit{type: enhancement''}\end{tabular}                 \\
P8B1        & \textit{``Labels that can define the type of the problem''}   \\
P11P1       & \textit{``The type of the programming language''}     \\ 
\hline
\end{tabular}
\end{table}

==> tables/label_typesOld.tex <==
\begin{table}[h]
 \begin{center}
 \caption{Quotations about the API labels Types}
 \label{tab:labelTypes}
 \begin{tabular}{c|c} 
  \hline
  \textbf{Participant} & \textbf{Quotation} \\
  \hline
 P9B1 & ``One that indicates that the issue is critical/important, and labels related to technologies/frameworks/libs involved''  \\
  
P7B1 & ``Maybe an information about programming language or if it is related to frontend, backend or database'' \\

P10P1 & ``impact on operations.''  \\

P3B1 & ``I thought it's important to only put relevant'' labels on the issues, 'cause improving the number of label could make them less readable.''  \\

P12B0 & ``type: performance, type: feature, API: User Interface and type: enhancement''  \\

P8B1 & ``Labels that can define the type of the problem'' \\

P11P1 & ``The type of the programming language'' \\

\hline
	
 \end{tabular}
 \end{center}
\end{table}

==> tables/reason_open.tex <==
 \begin{table}[]
 \caption{Quotations about reason to select the API labels}
 \label{tab:reason_Open}
\begin{tabular}{c|l}
\hline
Participant & \multicolumn{1}{c}{Quotation} \\
  \hline 
P5B0        & \textit{``[Labels] give a good idea of what the issue is about''}                        \\
P4B0        & \begin{tabular}[c]{@{}l@{}}\textit{``The labels were useful to know the problem area and }\\ \textit{after reading the title of the issues, it was the first thing }\\ \textit{[the participant]
taken into consideration, even }\\ \textit{ before opening to check the details''}
\end{tabular}                                         \\
P13I0       & \textit{``Quick identify what issue is related to''}              \\
P13B0        & \textit{``[Labels are] visual hints about it's classification''} \\
P14B0       & \begin{tabular}[c]{@{}l@{}}\textit{``[Labels are] hints about what areas have connection with}  \\ \textit{the problem occurring''}\end{tabular}                 \\

\hline
\end{tabular}
\end{table}

==> tables/reasons_regions.tex <==
\begin{table}[htb]
\centering
\caption{Reasons presented by participants to consider the region of information from the issue's page as relevant to decide about selecting the issue}
\label{tab:reasons_regions}
\begin{tabular}{|l|l|}
\hline
\textbf{Reasons}      & \textbf{Regions from the Issue's Page}                      \\ \hline
\begin{tabular}[c]{@{}l@{}}Information \\ about the issue\end{tabular}       & \begin{tabular}[c]{@{}l@{}}Title, Labels, Body, \\ Comments, Code Snipped\end{tabular} \\ \hline
Type of the issue     & Labels                                \\ \hline
Scenario of the issue & Linked Issue, Comments                \\ \hline
Localize the issue    & Code Snippet                          \\ \hline
Connected areas       & Linked Issue, Comments                \\ \hline
Start Point           & Body, Comments, Code Snippet          \\ \hline
Previous Attempts     & Comments, Linked Issue                \\ \hline
Steps to Reproduce    & Body, Comments                        \\ \hline
Steps to Debug        & Comments                              \\ \hline
Challenges faced      & Comments                              \\ \hline
Expected behaviour    & Title, Body, Comments                 \\ \hline
Suggested solutions   & Comments                              \\ \hline
Required skills       & Title, Labels                           \\ \hline
Experience level      & Title, Body, Comments                 \\ \hline
Feeling Safe          & Body, Comments                        \\ \hline
Easy to Work          & Title                                 \\ \hline
Getting Attracted     & Title, Labels, Body, Comments, Status \\ \hline
Required effort       & Title, Body                           \\ \hline
Status open or closed & Labels, Status                        \\ \hline
\begin{tabular}[c]{@{}l@{}}Description of an\\ ongoing solution\end{tabular} & Comments                                                                               \\ \hline
\end{tabular}
\end{table}


==> tables/regionsResults.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Why the information you selected was useful?}
 \label{tab:regionsResults}
\begin{tabular}{lll}
\cline{1-1} \cline{3-3}
\multicolumn{1}{|l|}{\textbf{What is the issue}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Where is the issue}} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{About} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Localize the issue} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Type} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Connected areas} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Goal} &  &  \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Benefits} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Why is an issue}} \\ \cline{1-1} \cline{3-3} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Goal} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{\textbf{How to solve the issue}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Benefits} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Start Point} &  &  \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Previous Attempts} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Who will solve the issue}} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Reproducing Steps} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Required skills} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Debug} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Difficulty level} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Challenges} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Required effort} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Expected behaviour} &  &  \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Suggested solutions} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\textbf{Motivation to work on the issue}} \\ \cline{1-1} \cline{3-3} 
\textbf{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Safe} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{\textbf{The issue status}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Easy} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Tag open/closed} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Attraction} \\ \cline{1-1} \cline{3-3} 
\multicolumn{1}{|l|}{Description of ongoing solution} &  &  \\ \cline{1-1}
\end{tabular}
\end{table}

==> tables/resultsFRFM_old.tex <==
\begin{table}[h!]
 \begin{center}
 \caption{overall metrics from models created to evaluate the corpus}
 \label{tab:results}
 \begin{tabular}{c|r|r|r|r} 
  \hline

  \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} &
  \textbf{Hla} \\
  \hline
Title (T) &	0.655 &	0.628 &	0.641 &	0.172 \\
Body (B)&	0.662 &	0.608 &	0.634 &	0.175 \\
T, B &	0.663 &	0.606 &	0.630 &	0.172 \\
T, B, Comments &	0.659 &	0.618 &	0.633 &	0.176 \\
 \hline

 \end{tabular}
 \end{center}
\end{table}

==> tables/surveyDemo.tex <==
\begin{table}[h!]
 \begin{center}
 \caption{Demographics Subgroups for the Experiment's Participants}
 \label{tab:results}
 \begin{tabular}{c|r|r|r|r} 
  \hline

  \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} &
  \textbf{Hla} \\
  \hline
Title (T) &	0.655 &	0.628 &	0.641 &	0.172 \\
Body (B)&	0.662 &	0.608 &	0.634 &	0.175 \\
T, B &	0.663 &	0.606 &	0.630 &	0.172 \\
T, B, Comments &	0.659 &	0.618 &	0.633 &	0.176 \\
 \hline

 \end{tabular}
 \end{center}
\end{table}

==> tables/survey_demo.tex <==
\begin{table}[htb]
\centering
\caption{Demographics Subsets for the Experiment's Participants}
\label{tab:demographics}

\begin{tabular}{lllllll}
\cline{1-3} \cline{5-7}
\multicolumn{1}{|l|}{Role}                                                               & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience with \\ JabRef technology\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Practitioner}                                                       & \multicolumn{1}{l|}{41} & \multicolumn{1}{l|}{55.5} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{High Experience}                                                              & \multicolumn{1}{l|}{31} & \multicolumn{1}{l|}{42}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Student}                                                            & \multicolumn{1}{l|}{33} & \multicolumn{1}{l|}{44.5} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Low Experience}                                                               & \multicolumn{1}{l|}{43} & \multicolumn{1}{l|}{58}   \\ \cline{1-3} \cline{5-7} 
                                                                                         &                         &                           &                       &                                                                                                 &                         &                           \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ Coder\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ OSS Contributor\end{tabular}}   & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Experienced}                                                        & \multicolumn{1}{l|}{28} & \multicolumn{1}{l|}{38}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Experienced}                                                                & \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{13.5} \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Novice}                                                             & \multicolumn{1}{l|}{46} & \multicolumn{1}{l|}{62}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Novice}                                                                     & \multicolumn{1}{l|}{64} & \multicolumn{1}{l|}{86.5} \\ \cline{1-3} \cline{5-7} 
\end{tabular}
\end{table}

==> tables/survey_demoT.tex <==
\begin{table}[htb]
\centering
\caption{Demographics Subsets for the Experiment's Participants}
\label{tab:demographics}

\begin{tabular}{lllllll}
\cline{1-3} \cline{5-7}
\multicolumn{1}{|l|}{Role}                                                               & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience with \\ JabRef technology\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Practitioner}                                                       & \multicolumn{1}{l|}{23} & \multicolumn{1}{l|}{56.1} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{High Experience}                                                              & \multicolumn{1}{l|}{17} & \multicolumn{1}{l|}{41.5}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Student}                                                            & \multicolumn{1}{l|}{18} & \multicolumn{1}{l|}{43.9} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Low Experience}                                                               & \multicolumn{1}{l|}{24} & \multicolumn{1}{l|}{58.5}   \\ \cline{1-3} \cline{5-7} 
                                                                                         &                         &                           &                       &                                                                                                 &                         &                           \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ Coder\end{tabular}} & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Experience as \\ OSS Contributor\end{tabular}}   & \multicolumn{1}{l|}{\#} & \multicolumn{1}{l|}{\%}   \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Experienced}                                                        & \multicolumn{1}{l|}{11} & \multicolumn{1}{l|}{26.8}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Experienced}                                                                & \multicolumn{1}{l|}{4} & \multicolumn{1}{l|}{9.8} \\ \cline{1-3} \cline{5-7} 
\multicolumn{1}{|l|}{Novice}                                                             & \multicolumn{1}{l|}{30} & \multicolumn{1}{l|}{73.2}   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Novice}                                                                     & \multicolumn{1}{l|}{37} & \multicolumn{1}{l|}{90.2} \\ \cline{1-3} \cline{5-7} 
\end{tabular}
\end{table}

==> tables/survey_demo_old.tex <==
\begin{table}[htb]
\centering
\caption{Demographics Subgroups for the Experiment's Participants}
\label{tab:demographics}
\begin{tabular}{lrrllrr}
\cline{1-3} \cline{5-7}
Role     & \multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} &  & Role              & \multicolumn{1}{l}{\#} & \multicolumn{1}{l}{\%} \\ \cline{1-3} \cline{5-7} 
Industry Practitioner & 41                     & 55.5                   &  & Experienced Coder & 19                     & 25.7                     \\
Student  & 33                     & 44.5                   &  & Novice Coder      & 55                     & 74.3                     \\ \cline{1-3} \cline{5-7} 
\end{tabular}
\end{table}
